The Bitter Lesson Learned from 2,000+ Multilingual Benchmarks

As large language models (LLMs) continue to advance in linguistic capabilities, robust multilingual evaluation has become essential for promoting equitable technological progress. This position paper examines over 2,000 multilingual (non-English) benchmarks from 148 countries, published between 2021 and 2024, to evaluate past, present, and future practices in multilingual benchmarking. Our findings reveal that, despite significant investments amounting to tens of millions of dollars, English remains significantly overrepresented in these benchmarks. Additionally, most benchmarks rely on original language content rather than translations, with the majority sourced from high-resource countries such as China, India, Germany, the UK, and the USA. Furthermore, a comparison of benchmark performance with human judgments highlights notable disparities. STEM-related tasks exhibit strong correlations with human evaluations (0.70 to 0.85), while traditional NLP tasks like question answering (e.g., XQuAD) show much weaker correlations (0.11 to 0.30). Moreover, translating English benchmarks into other languages proves insufficient, as localized benchmarks demonstrate significantly higher alignment with local human judgments (0.68) than their translated counterparts (0.47). This underscores the importance of creating culturally and linguistically tailored benchmarks rather than relying solely on translations. Through this comprehensive analysis, we highlight six key limitations in current multilingual evaluation practices, propose the guiding principles accordingly for effective multilingual benchmarking, and outline five critical research directions to drive progress in the field. Finally, we call for a global collaborative effort to develop human-aligned benchmarks that prioritize real-world applications.

==> figures/affiliations.tex <==
\begin{figure*}
\centering
\includegraphics[width=0.9\linewidth]{figures/institutions.pdf}
\caption{
Affiliation type distribution by country. We merge the European Union countries for better visualization.
}
\label{fig:affiliations}
\end{figure*}

% European Union {'Academic': 575, 'Industry': 20, 'Hybrid': 180}
% China {'Academic': 243, 'Industry': 45, 'Hybrid': 170}
% USA {'Academic': 265, 'Industry': 38, 'Hybrid': 149}
% UK {'Academic': 108, 'Industry': 7, 'Hybrid': 48}
% India {'Academic': 108, 'Industry': 8, 'Hybrid': 43}
% Canada {'Academic': 51, 'Industry': 4, 'Hybrid': 42}
% South Korea {'Academic': 45, 'Industry': 7, 'Hybrid': 28}
% Japan {'Academic': 44, 'Industry': 6, 'Hybrid': 24}
% UAE {'Academic': 41, 'Industry': 1, 'Hybrid': 16}
% Russia {'Academic': 25, 'Industry': 3, 'Hybrid': 24}
% Bangladesh {'Academic': 40, 'Industry': 1, 'Hybrid': 10}
% Vietnam {'Academic': 34, 'Industry': 4, 'Hybrid': 7}
% Iran {'Academic': 40, 'Industry': 1, 'Hybrid': 1}
% Australia {'Academic': 27, 'Industry': 0, 'Hybrid': 12}
% Singapore {'Academic': 14, 'Industry': 1, 'Hybrid': 22}
% Brazil {'Academic': 27, 'Industry': 1, 'Hybrid': 8}
% Saudi Arabia {'Academic': 21, 'Industry': 2, 'Hybrid': 6}
% Israel {'Academic': 20, 'Industry': 0, 'Hybrid': 6}
% Indonesia {'Academic': 8, 'Industry': 2, 'Hybrid': 14}
% Turkey {'Academic': 15, 'Industry': 1, 'Hybrid': 6}
% Qatar {'Academic': 13, 'Industry': 0, 'Hybrid': 5}
% Nigeria {'Academic': 10, 'Industry': 0, 'Hybrid': 7}
% Ethiopia {'Academic': 8, 'Industry': 0, 'Hybrid': 7}
% Mexico {'Academic': 8, 'Industry': 0, 'Hybrid': 7}
% South Africa {'Academic': 8, 'Industry': 0, 'Hybrid': 5}
% Pakistan {'Academic': 13, 'Industry': 0, 'Hybrid': 0}
% Sri Lanka {'Academic': 11, 'Industry': 0, 'Hybrid': 1}
% Egypt {'Academic': 5, 'Industry': 0, 'Hybrid': 5}
% Philippines {'Academic': 6, 'Industry': 0, 'Hybrid': 3}
% Uganda {'Academic': 2, 'Industry': 0, 'Hybrid': 6}
% Thailand {'Academic': 3, 'Industry': 1, 'Hybrid': 4}


% import matplotlib.pyplot as plt
% import geopandas as gpd
% import numpy as np
% from matplotlib.patches import Circle, Wedge
% import pandas as pd
% from matplotlib.colors import to_rgba
% import json
% from collections import Counter
% import math

% def read_jsonl(filename):
%     lst = []
%     with open(filename, "r") as f:
%         for line in f.readlines():
%             dic = json.loads(line.strip())
%             lst.append(dic)
%     return lst


% def main():
%     # Load world map
%     world = gpd.read_file(gpd.datasets.get_path("naturalearth_lowres"))

%     # Institution types
%     institution_types = {
%         "academic": "Academic",
%         "industry": "Industry",
%         "combined": "Hybrid",
%         "academic and industry": "Hybrid",
%         "academic, industry": "Hybrid",
%         "academic and non-profit": "Hybrid",
%     }
%     institution_keys = ["Academic", "Industry", "Hybrid"]

%     # ISO_a3 code for countries
%     country_code_map = {
%         "China": "CHN",
%         "USA": "USA",
%         "Germany": "DEU",
%         "UK": "GBR",
%         "India": "IND",
%         "Canada": "CAN",
%         "France": "FRA",
%         "South Korea": "KOR",
%         "Japan": "JPN",
%         "Spain": "ESP",
%         "UAE": "ARE",
%         "Russia": "RUS",
%         "Bangladesh": "BGD",
%         "Denmark": "DNK",
%         "Italy": "ITA",
%         "Vietnam": "VNM",
%         "Switzerland": "CHE",
%         "Iran": "IRN",
%         "Australia": "AUS",
%         # Use Malaysia as a placeholder for "Singapore" in the data
%         "Singapore": "MYS",
%         "Brazil": "BRA",
%         "Netherlands": "NLD",
%         "Finland": "FIN",
%         "Poland": "POL",
%         "Sweden": "SWE",
%         "Saudi Arabia": "SAU",
%         "Israel": "ISR",
%         "Indonesia": "IDN",
%         "Turkey": "TUR",
%         "Slovenia": "SVN",
%         "Czech Republic": "CZE",
%         "Portugal": "PRT",
%         "Belgium": "BEL",
%         "Ireland": "IRL",
%         "Nigeria": "NGA",
%         "Qatar": "QAT",
%         "Romania": "ROU",
%         "Norway": "NOR",
%         "Ethiopia": "ETH",
%         "Mexico": "MEX",
%         "South Africa": "ZAF",
%         "Pakistan": "PAK",
%         "Sri Lanka": "LKA",
%         "Greece": "GRC",
%         "Egypt": "EGY",
%         "Uganda": "UGA",
%         "Slovakia": "SVK",
%         "Austria": "AUT",
%         "Philippines": "PHL",
%         "Thailand": "THA",
%     }
%     country_code_map_rev = {v: k for k, v in country_code_map.items()}

%     # Read data
%     data = read_jsonl("/mnt/nas/minghaowu/marcoeval-project/globalbench/positions_scripts/metadata_new_20250320_tasks_keywords_institutions_yearmonth_country.jsonl")

%     countries = []
%     for item in data:
%         countries += item["country"]
%     countries = [c for c in countries if c != "NA"]
%     # print(Counter(countries).most_common(50))
%     country_freq = Counter(countries).most_common(50)
%     country_names = [c[0] for c in country_freq]
    
%     pie_data = {}
%     for country_name in country_names:
%         paper_lst = [i for i in data if country_name in i["country"]]
%         inst_types = [institution_types[i["institution_type"]] for i in paper_lst]
%         inst_freq = Counter(inst_types)
%         pie_data[country_code_map[country_name]] = [inst_freq.get(k, 0) for k in institution_keys]


%     # European Union
%     euro_data = {}
%     for i, row in world.iterrows():
%         country_code = row["iso_a3"]
%         continent = row["continent"]
%         if country_code in pie_data and continent == "Europe" and country_code != "GBR" and country_code != "RUS":
%             euro_data[country_code] = pie_data.pop(country_code)

%     print(euro_data)
%     euro_academic = [v[0] for v in euro_data.values()]
%     euro_industry = [v[1] for v in euro_data.values()]
%     euro_hybrid = [v[2] for v in euro_data.values()]

    
%     # Use Germany as a placeholder for "EU" in the data
%     pie_data["DEU"] = [sum(euro_academic), sum(euro_industry), sum(euro_hybrid)]

%     # Sort by sum of values
%     pie_data = {k: v for k, v in sorted(pie_data.items(), key=lambda x: sum(x[1]), reverse=True)}

%     for k, v in pie_data.items():
%         if k == "DEU":
%             print("European Union", {"Academic": sum(euro_academic), "Industry": sum(euro_industry), "Hybrid": sum(euro_hybrid)})
%         else:
%             print(country_code_map_rev[k], {"Academic": v[0], "Industry": v[1], "Hybrid": v[2]})


%     print(pie_data)
%     # raise NotImplementedError("Please implement the main function.")
    
%     # Remove Antarctica
%     world = world[world["name"] != "Antarctica"]
    
%     # Create figure and axis
%     fig, ax = plt.subplots(1, 1, figsize=(15, 10))
    
%     # Remove frame boundary
%     ax.spines['top'].set_visible(False)
%     ax.spines['right'].set_visible(False)
%     ax.spines['bottom'].set_visible(False)
%     ax.spines['left'].set_visible(False)
%     ax.set_xticks([])
%     ax.set_yticks([])
    
%     # Plot world map
%     world.plot(ax=ax, color="lightgrey", edgecolor="white")
    
%     # Color scheme for pie segments
%     colors = ["#ff9999", "#66b3ff", "#99ff99"]
    
%     # Draw pie charts for countries
%     # Find maximum sum for normalization
%     max_sum = max([sum(values) for values in pie_data.values()]) if pie_data else 1
    
%     for idx, row in world.iterrows():
%         country_code = row["iso_a3"]

%         if country_code in pie_data:

%             country_name = row["name"]
%             if country_name == "United States of America":
%                 country_name = "USA"
%             elif country_name == "Germany":
%                 country_name = "EU"
%             elif country_name == "United Arab Emirates":
%                 country_name = "UAE"
%             elif country_name == "Malaysia":
%                 country_name = "Singapore"
%             elif country_name == "United Kingdom":
%                 country_name = "UK"

%             # Get country centroid
%             centroid = row["geometry"].centroid
            
%             # Set pie chart size based on sum of values
%             values_sum = sum(pie_data[country_code])
%             # Scale factor can be adjusted to change the overall size of pie charts
%             scale_factor = 3
%             pie_size = math.sqrt(values_sum / scale_factor)
            
%             # Draw pie chart
%             if country_name == "Singapore":
%                 draw_pie_chart(ax, centroid.x - 5, centroid.y, pie_data[country_code], 
%                            colors, size=pie_size)
%             else:
%                 draw_pie_chart(ax, centroid.x, centroid.y, pie_data[country_code], 
%                             colors, size=pie_size)
                
%             # Add country name
%             if country_name =="Singapore":
%                 ax.text(centroid.x - 5, centroid.y - pie_size - 3, country_name, 
%                    horizontalalignment='center', fontsize=8, fontweight='bold')
%             else:
%                 ax.text(centroid.x, centroid.y - pie_size - 3, country_name, 
%                     horizontalalignment='center', fontsize=8, fontweight='bold')
    
%     # Add legend
%     legend_labels = institution_keys # ["Category A", "Category B", "Category C"]
%     legend_patches = [plt.Rectangle((0, 0), 1, 1, fc=color) for color in colors]
%     ax.legend(legend_patches, legend_labels, loc="lower left")
    
%     # Set title and adjust layout
%     # plt.title("Affliation Types for Each Country")
%     plt.tight_layout()
%     plt.savefig("institutions.pdf")
%     plt.show()

% def draw_pie_chart(ax, x, y, sizes, colors, size=1):
%     """Draw a pie chart at the specified position."""
%     if not sizes:
%         return
    
%     total = sum(sizes)
    
%     # Convert to angles
%     angles = [s/total * 360 for s in sizes]
    
%     # Draw wedges
%     start_angle = 0
%     for i, angle in enumerate(angles):
%         wedge = Wedge((x, y), size, start_angle, start_angle + angle, 
%                       fc=colors[i % len(colors)], alpha=0.8, edgecolor="white", linewidth=0.5)
%         ax.add_patch(wedge)
%         start_angle += angle

% if __name__ == "__main__":
%     main()



==> figures/size_distribution.tex <==
% \begin{figure}[]
%     \centering
%     \includegraphics[width=0.5\linewidth]{figures/size_distribution.pdf}
%     \caption{Distribution of multilingual benchmarks by dataset size from 2021 to 2024. Categories include very large (>100,000 examples), large (10,000-100,000), medium (1,000-10,000), small (100-1,000), and very small (<100) datasets.}
%     \label{fig:size_distribution}
% \end{figure}

% years = ["2021", "2022", "2023", "2024"]

% categories = [
%     ">100000",
%     "10000-100000",
%     "1000-10000",
%     "100-1000",
%     "<100"
% ]

% values = [
%     [104, 155, 204, 304],  # >100000
%     [82, 94, 110, 181],    # 10000-100000
%     [72, 90, 141, 228],    # 1000-10000
%     [39, 34, 73, 102],     # 100-1000
%     [1, 1, 1, 8]           # <100
% ]


\begin{figure*}[t]
\centering          
\subfigure[Task Trend]{\label{fig:tasks_trend}\includegraphics[scale=0.8]{figures/tasks_trend1.pdf}} 
\subfigure[Size Distribution]{\label{fig:size_distribution}\includegraphics[scale=0.8]{figures/size_distribution1.pdf}} 
\caption{(a) Evolution of popularity for the top 5 NLP tasks from 2021 to 2024. TC: text classification; QA: question answering; NER: named entity recognition; MRC: machine reading comprehension; SA: sentiment analysis. (b) Distribution of multilingual benchmarks by dataset size from 2021 to 2024. Categories include very large (>100,000 examples), large (10,000-100,000), medium (1,000-10,000), small (100-1,000), and very small (<100) datasets..}
\end{figure*}


% import matplotlib.pyplot as plt
% import numpy as np
% from matplotlib.font_manager import FontProperties

% # Data
% years = ["2021", "2022", "2023", "2024"]
% categories = [
%     ">100000",
%     "10000-100000",
%     "1000-10000",
%     "100-1000",
%     "<100"
% ]
% values = [
%     [104, 155, 204, 304],  # >100000
%     [82, 94, 110, 181],    # 10000-100000
%     [72, 90, 141, 228],    # 1000-10000
%     [39, 34, 73, 102],     # 100-1000
%     [1, 1, 1, 8]           # <100
% ]

% fig, ax = plt.subplots(figsize=(4,4))

% title_font = FontProperties(weight='bold', size=16)
% label_font = FontProperties(size=9)
% value_font = FontProperties(size=10)

% colors = ['#516b91','#59c4e6','#edafda','#93b7e3','#a5e7f0']

% x = np.arange(len(years))  
% bar_width = 0.6
% bottoms = np.zeros(len(years))

% for i, category_values in enumerate(values):
%     bars = ax.bar(x, category_values, bottom=bottoms, width=bar_width, 
%                  label=categories[i], color=colors[i])
%     bottoms += category_values

% ax.set_xlabel('Year')
% ax.set_ylabel('Value')

% ax.set_xticks(x)
% ax.set_xticklabels(years, fontproperties=label_font)
% legend = ax.legend(prop=label_font, loc='upper center', bbox_to_anchor=(0.5, -0.13),ncol=3)

% for label in ax.get_yticklabels():
%     label.set_fontproperties(label_font)


% ax.spines['top'].set_visible(False)
% ax.spines['right'].set_visible(False)

% # Adjust layout
% plt.tight_layout()
% plt.savefig('/bask/homes/f/fksv3157/xngs6460-languages/weixuan/results/figures/dynsample/size_distribution1.pdf', dpi=600, bbox_inches='tight')

% # Show plot
% plt.show()



% import matplotlib.pyplot as plt
% import numpy as np
% import matplotlib.font_manager as font_manager

% bold_font = font_manager.FontProperties(weight='bold')

% years = [2021, 2022, 2023, 2024]
% tasks = ['TC','QA','NER','MRC','SA']
% percentages = np.array([
%     [43.62, 41.18, 43.29, 44.59],  # text classification
%     [14.43, 12.57, 27.60, 37.42],  # question answering
%     [30.87, 31.82, 26.47, 23.09],  # named entity recognition
%     [8.72, 11.23, 20.79, 27.70],   # machine reading comprehension
%     [20.13, 17.38, 20.04, 18.96],  # sentiment analysis
% ])

% fig, ax = plt.subplots(figsize=(4, 4))
% markers = ['o','s','^','d','X']
% colors = ['#516b91','#59c4e6','#edafda','#93b7e3','#a5e7f0']
% for i, task in enumerate(tasks):
%     plt.plot(years, percentages[i], marker=markers[i], linewidth=2.2, markersize=6, label=task,color=colors[i])

% plt.xlabel('Year')
% plt.ylabel('Performance (%)')
% plt.legend(loc='upper center', bbox_to_anchor=(0.5, -0.15), ncol=3,prop=bold_font)

% ax.spines['top'].set_visible(False)
% ax.spines['right'].set_visible(False)

% plt.xticks(years)
% plt.tight_layout()
% plt.savefig('/bask/homes/f/fksv3157/xngs6460-languages/weixuan/results/figures/dynsample/tasks_trend1.pdf', dpi=600, bbox_inches='tight')

% plt.show()

==> figures/translation_and_tasks.tex <==
\begin{figure*}[h!]
\centering          
\subfigure[Translations]{
\includegraphics[scale=0.2]{figures/translators1.png}
\label{fig:translations}
} 
\subfigure[Tasks]{
\includegraphics[scale=0.5]{figures/tasks_trend1.pdf}
\label{fig:tasks}
} 
\caption{
(a) Distribution of translation methods used in benchmark creation.
(b) Percentage distribution of top 5 tasks in multilingual benchmarks from 2021 to 2024. TC: Text Classification, NER: Named Entity Recognition, SA: Sentiment Analysis, QA: Question Answering, MRC: Machine Reading Comprehension.
}
\label{fig:translations_and_tasks}
\end{figure*}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> signlanguage.tex <==
QvQ-72B-preview

Answer

So I'm trying to figure out what number this hand sign represents in American Sign Language (ASL). Let me see... In ASL, each number from 0 to 10 has its own unique hand shape, and it's important to recognize them correctly.

First, I need to observe the hand position. The thumb is bent and touching the base of the index finger, and then the index, middle, and ring fingers are extended straight up. The pinky is also extended, but it seems like it might be slightly bent or not as straight as the other fingers. The palm is facing towards me.

Let me recall the ASL numbers. Starting from zero:

0: Fist, thumb touches the pinky.
1: Index finger extended, rest are closed.
2: Index and middle fingers extended.
3: Index, middle, and ring fingers extended.
4: Index, middle, ring, and pinky extended.
5: All fingers extended.
6: All fingers extended, thumb touches the side of the index finger.
7: All fingers extended, thumb crosses over to touch the middle finger.
8: All fingers extended, thumb touches the ring finger.
9: All fingers extended, thumb touches the pinky.
10: Both hands showing 5.
Looking at this, the hand has the thumb bent and touching near the index finger, and four fingers extended: index, middle, ring, and pinky. Wait, but in the description, it says the pinky is slightly bent. Maybe it's not fully extended like the other fingers.

In ASL, the number 4 is shown with all four fingers extended and the thumb touching the base of the index finger. That seems similar to what's being shown here. But I need to make sure.

Let me check again: thumb is bent and touching near the index finger, and the index, middle, ring, and pinky are extended. If the pinky is slightly bent, maybe it's still considered as extended for the purpose of the sign.

Alternatively, maybe it's the number 9, which also involves the thumb touching the pinky while all fingers are extended. But in 9, the thumb touches the pinky, whereas in 4, the thumb touches the base of the index finger.

Wait, according to the standard ASL hand shapes, number 4 is indeed the hand with the thumb touching the base of the index finger and the four fingers extended.

Number 9, on the other hand, has all five fingers extended with the thumb touching the pinky.

So, in the image, if the thumb is touching near the index finger and four fingers are extended, it should be the number 4 sign in ASL.

But I'm a bit confused because I thought in number 9, the thumb touches the pinky while all fingers are extended. Maybe the description is a bit unclear about the exact position of the thumb.

Let me try to visualize this again. Thumb is bent and touching the base of the index finger, and the index, middle, ring, and pinky are extended. That matches the description of number 4 in ASL.

Number 9 would have all five fingers extended, with the thumb touching the pinky, which isn't the case here since the thumb is touching the base of the index finger.

Therefore, the hand sign in the image represents the number 4 in American Sign Language.

Final Answer

4
4
​


==> tables/tasks.tex <==
\begin{table}[]
\begin{tabular}{lcccc}
                                & 2021  & 2022  & 2023  & 2024  \\
text classification           & 43.62 & 41.18 & 43.29 & 44.59 \\
question answering            & 14.43 & 12.57 & 27.60 & 37.42 \\
named entity recognition      & 30.87 & 31.82 & 26.47 & 23.09 \\
machine reading comprehension & 8.72  & 11.23 & 20.79 & 27.70 \\
sentiment analysis            & 20.13 & 17.38 & 20.04 & 18.96
\end{tabular}
\caption{The percentage of top 5 tasks from 2021 to 2024.}
\label{table:tasks}
\end{table}
